RAGIC: Risk-Aware Generative Adversarial Model for Stock Interval Construction

Efforts to predict stock market outcomes have yielded limited success due to the inherently stochastic nature of the market, influenced by numerous unpredictable factors. Many existing prediction approaches focus on single-point predictions, lacking the depth needed for effective decision-making and often overlooking market risk. To bridge this gap, we propose a novel model, RAGIC, which introduces sequence generation for stock interval prediction to quantify uncertainty more effectively. Our approach leverages a Generative Adversarial Network (GAN) to produce future price sequences infused with randomness inherent in financial markets. RAGIC's generator includes a risk module, capturing the risk perception of informed investors, and a temporal module, accounting for historical price trends and seasonality. This multi-faceted generator informs the creation of risk-sensitive intervals through statistical inference, incorporating horizon-wise insights. The interval's width is carefully adjusted to reflect market volatility. Importantly, our approach relies solely on publicly available data and incurs only low computational overhead. RAGIC's evaluation across globally recognized broad-based indices demonstrates its balanced performance, offering both accuracy and informativeness. Achieving a consistent 95% coverage, RAGIC maintains a narrow interval width. This promising outcome suggests that our approach effectively addresses the challenges of stock market prediction while incorporating vital risk considerations.

==> table/features.tex <==

\begin{table*}[!htbp]
    \centering\fontsize{9}{9}\selectfont
    \caption{Feature preprocessing. $x_t$ denotes the corresponding features before processing.}
    \begin{tabular}{c|c|c}
    \hline
    Type & Features & Calculation \\
    \hline
    \multirow{2}*{Price} & Open, Close, High, Low  &{$x_t/close_{t-1} -1$} \\
    \cline{2-3} & Volume & $x_t/x_{t-1} -1$\\
    \hline
    \multirow{6}*{Technical indicator} &  RSI & -1 if $x_t<20$, 1 if $x_t\geq 80$, 0 otherwise\\
    \cline{2-3} & MACD DIFF & min-max scaling \\
    \cline{2-3} & Upper Bollinger band indicator & 1 if $close_t>BOLU$, 0 otherwise \\
    \cline{2-3} & Lower Bollinger band indicator & 1 if $close_t<BOLD$, 0 otherwise \\
    \cline{2-3} & EMA: 5-day 
    &\multirow{2}*{$x_t/close_t - 1$}  \\ 
    \cline{2-2} &SMA: 13-day, 21-day, 50-day \\
    \hline
    \multirow{2}*{Volatility} & Volatility index & min-max scaling \\
    \cline{2-3} & Return of Volatility index & {$x_t/x_{t-1} -1$} \\ 
    \hline
    \end{tabular}
    \label{tab:feature}
\end{table*}


==> table/hyper_baselines.tex <==

\begin{table*}[!htbp]
    \centering\fontsize{9}
    {9}\selectfont
    \caption{Hyperparameters on baselines for the datasets.}
    \begin{tabular}{c|c|c|ccccc}
    \toprule Model & Parameter & Range  & DJI & SPX & Nasdaq & DAX & Nikkei  \\
    \midrule

    \multirow{2}*{Bollinger bands} & Sequence Length & 20 & \multicolumn{5}{c}{20} \\
    & Number of std & 2 & \multicolumn{5}{c}{2} \\  \hline
    
    \multirow{10}*{\thead{BayesianNN \\ MQRNN}} & Epochs & [30,300] & \multicolumn{5}{c}{50} \\
    & Learning rate & [0.0001,0.01] & \multicolumn{5}{c}{0.01} \\ 
    & Batch size & [32,256] & \multicolumn{5}{c}{100} \\
    & Steps in an epoch & [10,100] & \multicolumn{5}{c}{500} \\ 
    & Optimizer & Adam, RMSProp & \multicolumn{5}{c}{Adam} \\ 
    & Embedding size & [10,100] & \multicolumn{5}{c}{20}\\
    & Sequence Length & [5,40] & \multicolumn{5}{c}{30}\\ 
    & Prediction Horizon & [1,10] & \multicolumn{5}{c}{5}\\   
    & Dropout rate (BayesianNN) & [0,1] & \multicolumn{5}{c}{0.5}\\ 
    \hline
    
    \multirow{9}*{CFRNN} & Epochs & [100,1500] & \multicolumn{5}{c}{1000} \\
    & Learning rate & [0.0001,0.01] & \multicolumn{5}{c}{0.01} \\ 
    & Batch size & [32,256] & \multicolumn{5}{c}{100} \\
    & Steps in an epoch & [10,100] & \multicolumn{5}{c}{500} \\ 
    & Optimizer & Adam, RMSProp & \multicolumn{5}{c}{Adam} \\ 
    & Embedding size & [10,100] & \multicolumn{5}{c}{20}\\
    & Sequence Length & [5,40] & \multicolumn{5}{c}{30}\\ 
    & Prediction Horizon & [1,10] & \multicolumn{5}{c}{5}\\  
    & Correction factor & [1,5] & \multicolumn{5}{c}{1}\\  
    \hline    
    
    \multirow{4}*{StockGAN} 
    & Epochs & [30,100] & \multicolumn{5}{c}{50} \\ 
    & Learning rate & [0.0001,0.01] & \multicolumn{5}{c}{0.002} \\  
    & Batch size & [32,256] & \multicolumn{5}{c}{64} \\ 
    & Optimizer & Adam, RMSProp & \multicolumn{5}{c}{Adam} \\ 
    & Sequence Length & [5,40] & \multicolumn{5}{c}{30}\\ 
    & Layers & [1,4] & \multicolumn{5}{c}{2}\\ 
    & Dimension(layer1) & [10,500] & 72 & 72 & 100 & 100 & 100 \\ & Dimension(layer2) & [10,500] & 10 & 10 & 10 &30 & 30 \\ \hline

    \multirow{7}*{FactorVAE} & Epochs & [30,100] & \multicolumn{5}{c}{50} \\ 
    & Learning rate & [0.0001,0.01] & \multicolumn{5}{c}{0.001} \\
    & Batch size & [32,256] & \multicolumn{5}{c}{128} \\ 
    & Optimizer & Adam, RMSProp & \multicolumn{5}{c}{Adam} \\ 
    &Sequence Length & [5,40] & \multicolumn{5}{c}{30} \\
    &Number of head & [1,5] & \multicolumn{5}{c}{5} \\
    &Weight of KLD loss & [0,10] & \multicolumn{5}{c}{0.2} \\ &Embedding size & [50,1000] & 500 & 500 & 500 & 800 & 850 \\\hline

    \multirow{8}*{HMG-TF} & Epochs & [30,100] & \multicolumn{5}{c}{50} \\ 
    & Batch size & [32,256] & \multicolumn{5}{c}{256} \\ 
    & Optimizer & Adam, RMSProp & \multicolumn{5}{c}{Adam} \\ 
    &Sequence Length & [5,40] & \multicolumn{5}{c}{20} \\
    &Number of block & [1,5] & \multicolumn{5}{c}{3} \\
    & Learning rate & [0.0001,0.01] & 0.001 & 0.001 & 0.001 & 0.0005 & 0.0005  \\
    &Number of head & [1,5] & 2 & 2 & 2 & 4 & 4 \\
    & Weight of penalty loss & [0,1] & 0.05 & 0.05 & 0.05 & 0.02 & 0.02 \\ \hline

    \multirow{5}*{AdaRNN} & Epochs & [30,300] & \multicolumn{5}{c}{200} \\ 
    & Number of layer & [1,5] & \multicolumn{5}{c}{2} \\
    & Batch size & [32,512] & \multicolumn{5}{c}{256} \\ 
    & Optimizer & Adam, RMSProp & \multicolumn{5}{c}{Adam} \\
    & Weight of penalty & [0,1] & \multicolumn{5}{c}{0.5} \\ 
    & Learning rate & [0.00001,0.01] & \multicolumn{5}{c}{0.00005} \\
    & Hidden size & [30,200] & \multicolumn{5}{c}{64} \\
    
    \bottomrule 
    \end{tabular}
    \label{tab:baselines}
\end{table*}


==> table/hyperparameters.tex <==

\begin{table*}[!htbp]
    \centering\fontsize{9}{9}\selectfont
    \caption{Hyperparameters on \RAGIC for the datasets.}
    \begin{tabular}{c|c|ccccc}
    \toprule Parameter & Range  & DJI & SPX & Nasdaq & DAX & Nikkei  \\
    \midrule  
    Epochs & [30,300] & \multicolumn{5}{c}{50} \\
    Optimizer & Adam, RMSProp &\multicolumn{5}{c}{Adam} \\
    Learning rate of critic & [0.00001, 0.01] & \multicolumn{5}{c}{0.0002} \\
    $\xi$ & [0.001,0.01] & \multicolumn{5}{c}{0.01} \\
    $\alpha_l$ & 90\% & \multicolumn{5}{c}{90\%} \\
    $\alpha_u$ & 99.9\% &  \multicolumn{5}{c}{99.9\%} \\
    $\Delta \epsilon$ & 0.0001&  \multicolumn{5}{c}{0.0001} \\
    $N$ & 50 & \multicolumn{5}{c}{50} \\
    $\gamma$ & [0.1,2] &  \multicolumn{5}{c}{0.3} \\
    $D$ & [2,4] &  \multicolumn{5}{c}{2}\\
    $\delta_k$ for volatility return & [0.05,0.25] & 0.1 & 0.05 & 0.2 & 0.1 & 0.1 \\
    $\delta_k$ for normalized volatility index & [0.05,0.25] &  0.25 & 0.05 & 0.1 & 0.05 & 0.2 \\
    $\lambda_k$ for volatility return & [0.5,4] & 2.5 & 1.5 & 2.5 & 1.5 & 1.5\\
    $\lambda_k$ for normalized volatility index & [0.5,4] & 1.5 & 1.5 & 4 & 2.5 & 2.5\\
    Batch size & [16,512] & 256 & 256&256&150&256 \\
    $n_{critic}$ & [2,6] & 4 & 4 & 3& 6& 5 \\
    Learning rate of generator & [0.00001, 0.05] & 0.0001 & 0.0001 & 0.00005 & 0.0001 & 0.0001  \\
    $L$ & [2,6] & 3 & 2 & 2 & 3 & 3\\
    $p$ &[2,8] & 8 & 5 & 5 & 8 & 8\\
    Dimension of hidden layer & [50, 300] & 150 & 100 & 100 & 150 & 150 \\
    $v_l$ & [10,20] & 10 & 10 & 10 & 12 & 10\\
    $v_u$ & [20,30] & 22  & 20 & 20 & 22 & 25 \\
    \bottomrule 
    \end{tabular}    
    \label{tab:hyper}
\end{table*}


==> table/stat_data1.tex <==

\begin{table}[!htp]
    \centering\fontsize{9}{9}\selectfont
    \caption{Statistics of stock indices.}
    \begin{tabular}{cccccc}
    \toprule 
    & DJI & SPX & Nasdaq & DAX & Nikkei\\
    \midrule  
    Volatility & VXD & VIX & VXN & VDAX & JNIV \\
    \# days & 6051 & 6051 & 5269 & 5237 & 4791\\
    start year & 1997 & 1997 & 2001 & 2001 & 2002\\
    \bottomrule 
    \end{tabular}
    
    \label{tab: dataset}
\end{table}



